Informative Path Planning with Limited Adaptivity

We consider the informative path planning ($\mathtt{IPP}$) problem in which a robot interacts with an uncertain environment and gathers information by visiting locations. The goal is to minimize its expected travel cost to cover a given submodular function. Adaptive solutions, where the robot incorporates all available information to select the next location to visit, achieve the best objective. However, such a solution is resource-intensive as it entails recomputing after every visited location. A more practical approach is to design solutions with a small number of adaptive "rounds", where the robot recomputes only once at the start of each round. In this paper, we design an algorithm for $\mathtt{IPP}$ parameterized by the number $k$ of adaptive rounds, and prove a smooth trade-off between $k$ and the solution quality (relative to fully adaptive solutions). We validate our theoretical results by experiments on a real road network, where we observe that a few rounds of adaptivity suffice to obtain solutions of cost almost as good as fully-adaptive ones.

==> tables/road_rac_table.tex <==
\begin{table}[H]
\centering
\caption{Relative Average Cost (vs. Fully Adaptive) for Road Networks}
\label{tab:road_rac}
\begin{tabular}{lrrrrrrrrrrr}
\toprule
 & \multicolumn{11}{c}{Relative Average Cost (vs. Fully Adaptive)} \\
Number of Rounds & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & inf \\
Problem Name &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
road-60-50 & 38.32 & 0.60 & -14.10 & -8.57 & -15.93 & -6.07 & -1.43 & -1.05 & 7.16 & -9.67 & 0.00 \\
road-60-50-2 & 7.46 & -23.66 & -18.49 & -23.91 & -17.36 & -15.04 & -15.76 & -12.90 & -6.60 & -19.64 & 0.00 \\
road-62-50 & 33.60 & 19.51 & 14.42 & 16.68 & 22.68 & 26.18 & 22.66 & 19.76 & 16.10 & 15.54 & 0.00 \\
road-62-50-2 & 9.54 & -24.07 & -18.78 & -17.86 & -0.68 & -3.52 & 7.14 & -5.30 & 17.42 & -2.94 & 0.00 \\
road-64-50 & 10.96 & 10.82 & 7.86 & 4.01 & 16.01 & 8.31 & 14.96 & 4.33 & 4.82 & 5.84 & 0.00 \\
road-64-50-2 & 5.32 & 6.59 & 8.72 & 5.50 & 13.77 & 30.35 & 22.82 & 33.05 & 4.61 & 21.46 & 0.00 \\
road-66-50 & 52.34 & 13.06 & 16.94 & 11.18 & 15.60 & 12.12 & 21.34 & -8.54 & -1.12 & -3.27 & 0.00 \\
road-66-50-2 & 30.02 & -26.60 & -17.55 & -9.54 & -18.90 & -11.06 & 5.91 & -11.52 & -4.15 & -5.87 & 0.00 \\
road-68-50 & 74.34 & 9.07 & 5.33 & 14.86 & 3.00 & -11.93 & 7.85 & -11.88 & -19.16 & -8.21 & 0.00 \\
road-68-50-2 & 88.94 & 25.84 & 23.97 & 3.32 & -8.35 & 12.10 & 4.33 & 19.24 & 31.30 & 28.97 & 0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/uav_rac_table.tex <==
\begin{table}[H]
\centering
\caption{Relative Average Cost (vs. Fully Adaptive) for UAV Search}
\label{tab:uav_rac}
\begin{tabular}{lrrrrrrrr}
\toprule
 & \multicolumn{8}{c}{Relative Average Cost (vs. Fully Adaptive)} \\
Number of Rounds & 1 & 2 & 3 & 4 & 5 & 6 & 7 & inf \\
Problem Name &  &  &  &  &  &  &  &  \\
\midrule
uav-8 & 57.61 & 13.76 & 10.35 & 6.51 & 12.84 & 16.22 & 13.63 & 0.00 \\
uav-8-OC & 86.84 & 4.67 & -1.97 & -6.12 & -0.89 & -5.88 & -2.16 & 0.00 \\
uav-9 & 52.48 & 11.30 & 1.53 & 0.82 & -0.28 & 1.18 & 7.18 & 0.00 \\
uav-9-OC & 68.90 & -6.51 & -1.19 & -3.86 & -0.03 & 1.06 & -2.19 & 0.00 \\
uav-10 & 81.67 & 5.21 & 5.21 & 4.08 & 3.04 & 0.14 & 1.91 & 0.00 \\
uav-10-OC & 100.07 & 10.03 & 8.33 & 6.71 & 5.16 & 4.01 & 5.12 & 0.00 \\
\bottomrule
\end{tabular}
\end{table}

